MMA-SafetyBench: A Benchmark for Multimodal Agent Safety Evaluation

Multimodal agents increasingly rely on visual interfaces to perceive state and select actions, creating an attack surface not captured by text-only safety evaluations. We study Visual Semantic Hijacking, in which deceptive but semantically meaningful interface elements, such as forged system alerts, cause an agent to depart from its authorized task. We propose a trajectory-guided procedure that identifies candidate injection points and inserts reproducible visual payloads into the observation stream. Using this procedure, we construct MMA-SafetyBench, which contains 1,083 adversarial trajectories across web automation, desktop GUI control, mobile navigation, document understanding, and video processing. Across nine evaluated models, Attack Success Rate (ASR) reaches 87.96%, while Semantic Compromise Rate (SCR) reaches 98.09%. A 1--3--5 scoring scheme distinguishes target-matching outputs, semantic disruption without a target match, and successful preservation of the benign task. Controls covering all nine models and five domains show that attacks persist under neutral prompts. A safety-priority prompt lowers ASR without eliminating the failure mode.

==> authors.tex <==
\author{%
  \begin{tabular}{@{}c@{}}
    \fontsize{11}{14}\selectfont
    Yuke Wang$^{2*}$\quad Benlei Cui$^{1*}$\quad Shen Pang$^{2}$\quad Xuemei Dong$^{2\dagger}$\quad Longtao Huang$^{1}$ \\[3pt]
    \fontsize{11}{14}\selectfont
    Hui Xue$^{1}$\quad Yuwen Zhai$^{1}$\quad Junjie Li$^{1}$\quad Jingqun Tang$^{3}$\quad Haiwen Hong$^{1\dagger}$ \\[8pt]
    {\normalfont\small $^{1}$Yuvion Team, Alibaba Group} \\[2pt]
    {\normalfont\small $^{2}$Laboratory for Statistical Monitoring and Intelligent Governance of Common Prosperity,} \\
    {\normalfont\small School of Statistics and Data Science, Zhejiang Gongshang University} \\[2pt]
    {\normalfont\small $^{3}$Jinshengyuliang AI}
  \end{tabular}%
}

% Unnumbered author notes have no reserved footnote-marker indentation.
\newcommand{\authornotetext}[1]{\noindent#1}
% Place author notes below the first-page text, with the standard footnote rule.
\AddToHook{cmd/maketitle/after}{%
  \begingroup
  \renewcommand{\thefootnote}{}%
  \expandafter\let\csname @makefntext\endcsname\authornotetext
  \footnotetext{%
    \setlength{\parindent}{0pt}\raggedright
    \noindent $^{*}$Equal contribution.\quad $^{\dagger}$Corresponding authors.\par\vspace{2pt}
    \noindent\textit{Author contributions.} Yuke Wang performed the main experiments.
    Benlei Cui conceived the study, developed the methodology, and wrote the manuscript.
    Yuwen Zhai provided the data for the GUI tasks.%
  }%
  \endgroup
}

